MoE-Infinity: Efficient MoE Inference on Personal Machines with Sparsity-Aware Expert Cache

This paper presents MoE-Infinity, an efficient MoE inference system designed for personal machines with limited GPU memory capacity. The key idea for MoE-Infinity is that on personal machines, which are often single-user environments, MoE-based LLMs typically operate with a batch size of one. In this setting, MoE models exhibit a high degree of activation sparsity, meaning a small number of experts are frequently reused in generating tokens during the decode phase. Leveraging this idea, we design a sparsity-aware expert cache, which can trace the sparse activation of experts during inference and carefully select the trace that represents the sparsity pattern. By analyzing these selected traces, MoE-Infinity guides the replacement and prefetching of the expert cache, providing 3.1-16.7x per-token latency improvements over numerous state-of-the-art systems, including vLLM, Ollama, DeepSpeed and BrainStorm across various MoE models (DeepSeek and Mixtral) when handling different LLM tasks. MoE-Infinity's source code is publicly available at https://github.com/EfficientMoE/MoE-Infinity

==> sections/challenges.tex <==
\section{Expert Activation Awareness}
\label{sec:challenge}

\subsection{Key Observations}
\label{sec:design-intutions}

% We have the following key observations that motivate our design for improving offloading.


% \begin{table}[t]
%     \centering
%     \begin{tabular}{|l|rrrrrr|}
%     \hline
%         Model       & bs=1 & 2  & 4  & 8 & 16   & 32      \\
%     \hline
%         Switch%-128x0.2B  
%         & 1.2  & 1.8  & 2.7   & 3.9 & 5.6      & 7.8          \\
%         NLLB%-128x0.4B    
%         & 3.6  & 5.3  & 7.6   & 10.6& 14.7     & 19.9          \\
%         Arctic%-128x4B   
%         & 1.5  & 2.7  & 4.5    & 6.9& 10.2  &   14.5        \\
%         Mixtral%-8x7B     
%         & 25.0 & 42.9  & 66.0  & 86.4& 96.7 &   99.3           \\
%     \hline
%     \end{tabular}
%     \caption{Expert activation ratio (\%) over batch size (bs).}
%     \label{tab:activation-sparsity}
% \end{table}

\mypar{(1)~Highly selective activations imply low fetching traffic}
In serving scenarios, LLM serving systems often exhibit \emph{low expert activation ratios} with MoE models. Our findings reveal that models with 128 experts per layer activate fewer than 5\% of experts for a single request. In contrast, configurations like Mixtral, with eight experts per layer and top-2 activation, show 25\% activation for single requests .

The above data indicate low expert activation ratios during decoding. 
Similar observations for prefilling under single input request with varing length is demonstrated in~\cref{sec:appendix-observations}.
A strategy of fetching only active experts for inference—unlike current practices of fetching all potentially active experts—could cut data fetching traffic significantly. This approach might reduce traffic by up to 98.5\% in models like Arctic, NLLB, and Switch during decoding. 

% \begin{figure}[t]
%     \centering
%     % \includegraphics[page=3, height=1.5in, width=.88\linewidth, trim={0cm 2cm 0cm 0cm},clip]{figures/illustration/overviews.pdf}
%     % \includegraphics[width=.9\linewidth]{figures/illustration/ conditional_activation_2.pdf}
%     \begin{subfigure}[h]{\linewidth}
%         \centering
%         \includegraphics[width=.8\linewidth]{figures/illustration/group_activation.pdf}
%         \caption{Example of intra-sequence group expert activation. The edge denotes the conditional activation count between a pair of experts. The higher the count, the wider the edge. We show the top hitter experts in each layer.}
%         \label{fig:conditional-activation}
%     \end{subfigure}
%     % \hfill
%     % \begin{subfigure}[h]{.48\linewidth}
%     %     \centering
%     %     \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_conditioning_single_snowflake_mmlu.png}
%     %     \caption{\review{Example of inter-sequence group expert activation, considering only single layer.}}
%     %     \label{fig:group-activation-single}
%     % \end{subfigure}
%     % \begin{subfigure}[h]{.48\linewidth}
%     %     \centering
%     %     \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_conditioning_snowflake_mmlu.png}
%     %     \caption{\review{Example of inter-sequence group expert activation, considering all layers from beginning.}}
%     %     \label{fig:group-activation-hist}
%     % \end{subfigure}
%     \caption{\review{Expert group activation for intra-sequence and inter-sequence.}}
%     \label{fig:activation}
% \end{figure}


\mypar{(2)~Group activation can facilitate prefetching}
In serving MoE models, we observe that a group of experts across multiple layers is often activated together. This observation is essentially attributed to the training method of MoE models~\cite{mixtral}, where a specialized group of experts is trained to process tokens, ensuring that fewer parameters are activated compared to their dense counterparts.

\begin{comment}
\review{
% need to say two things: 1) accounting for single expert + next layer cotrrelation is wrong; 2) layer activation as a group shows predictability.
We observe that effective group activation for prefetching requires consideration of patterns across all inference layers. To analyze this predictability, we assume the presence of a trace with similar activation patterns and demonstrate our findings using the Snowflake and MMLU datasets, with Pearson correlation as the metric. Similar trends are observed in models like NLLB, Switch, and Mixtral, as well as other datasets.
Our analysis considers two scenarios for each sequence: (i) prediction is based on the current MoE layer running inference, which often used in existing approaches~\cite{brainstorm,deepum} (in Figure~\ref{fig:group-activation-single}), 
and (ii) prediction is based on all activation collected from the first layer (in Figure~\ref{fig:group-activation-hist}).
In both scenarios, we observe that higher similarity in activation sequences during earlier layers strongly correlates with higher similarity in subsequent layers. Ideally, the distribution of points should exhibit low variance (indicating high precision in prefetching) and be bounded below by the black line (indicating high prefetching accuracy).
Figure~\ref{fig:group-activation-hist} demonstrates that multi-layer-based prediction aligns closer to the ideal case, offering improved precision and accuracy over single-layer-based methods.
% Viewing expert activation in each layer as a group, we find that higher similarity between activation sequences in earlier layers strongly correlates with higher similarity in later layers. This relationship holds for both initial layers (e.g., $l=2$) and deeper layers near the end (e.g., $l=33$).
% Specifically, we investigate whether the similarity between the current activation pattern (from layer 0 to layer $l$) and a previously observed pattern implies similarity in subsequent layers (from layer $l$ onwards).
% We further analyse the predictability of the expert activation.
% We aim to demonstrate the predictability in the following form as an interpolation:
% given expert activation pattern (including both sparse activation and activation counts) that has been observed, if current activation pattern from layer 0 to $l$ is similar to any one observation, than these two patterns are also similar in following layers from $l$ and onwards.
% Figure~\ref{fig:group-activation} shows the validation using Snowflake and MMLU dataset using Pearson correlation. 
% Similar pattern has also been observed on NLLB, Switch and Mixtral.
% When viewing the expert activation in each layer as a group, we observe that the higher the similarity between two sequences in group activation, the higher the similarity for future layers.
% And this can be generalized for both layers at the beginning (l=2) and layers approaching the end (l=33). 
% Figure~\ref{fig:group-activation-hist} shows that a similar activation pattern can be matched in trace, the deeper the layer, the higher the accuracy and precision of prefetching can be using the trace.
% Figure~\ref{fig:group-activation-single} shows the case for  where the routing information of the current layer of MoE model processing is used for prefetching. 
}
\end{comment}


\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/illustration/group_activation.pdf}
    \caption{Example of intra-sequence group expert activation. The edge denotes the conditional activation count between a pair of experts. The higher the count, the wider the edge. We show the top hitter experts in each layer.}
    \label{fig:conditional-activation}
\end{figure}

Figure~\ref{fig:conditional-activation} demonstrates group activation patterns in Switch.
The pattern is also observed in NLLB, Arctic, and Mixtral.
For instance, activating Expert 81 in Layer 0 (E[0,81]) is linked to higher activations of E[1,65], E[1,72], and E[1,81] in Layer 1. This pattern, indicating a cross-layer activation group like \{E[0,81], E[1,65], E[2,72]\}, suggests interconnected expert activations across layers. Different groups, e.g., \{E[0,81], E[1,72], E[2,72]\}, co-exist and show varied token traffic. For instance, \{E[0,81], E[1,72], E[2,62]\} experiences higher token traffic compared to \{E[0,81], E[1,81], E[2,21]\}.

Leveraging group activation patterns in MoE models can significantly enhance prefetching in MoE offloading systems. With experts holding up to hundreds of megabytes and GPU inference times mirroring PCIe data fetch times (both approximately 1 millisecond), overlapping prefetching and inference become feasible. By tracking active experts and employing historical group activation, the system can predict and prefetch the experts likely needed for subsequent layers.

\begin{figure}[t]
    \centering
    % \begin{subfigure}[h]{.32\linewidth}
    % \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_counts_heatmap_mixtral_mmlu_0.pdf}
    % \end{subfigure}
    % \begin{subfigure}[h]{.32\linewidth}
    % \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_counts_heatmap_mixtral_mmlu_3.pdf}
    % \end{subfigure}
    % \begin{subfigure}[h]{.32\linewidth}
    % \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_counts_heatmap_mixtral_mmlu_agg.pdf}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[h]{.32\linewidth}
    % \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_counts_heatmap_nllb_bigbench_0.pdf}
    % \end{subfigure}
    % \begin{subfigure}[h]{.32\linewidth}
    % \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_counts_heatmap_nllb_bigbench_3.pdf}
    % \end{subfigure}
    % \begin{subfigure}[h]{.32\linewidth}
    % \includegraphics[width=\linewidth]{figures/illustration/decoder_layer_counts_heatmap_nllb_bigbench_agg.pdf}
    % \end{subfigure}
    \includegraphics[width=\linewidth]{figures/illustration/reuse_hist_mixtral.pdf}
    \includegraphics[width=\linewidth]{figures/illustration/reuse_hist_nllb.pdf}
    \caption{Expert reuse count over 20 decoding iterations for two sample sequences and merged over 1000 sequences. Darker colour means higher reuse normalized. Sampled from last layer of Mixtral-8x7B (top) and NLLB-128x1B (bottom).\cs{Todo: make the correlation more clear}}
    \label{fig:expert-reused}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/illustration/merged_reuse.pdf}
%     \caption{Expert reuse count merged over 1000 sequences.}
%     \label{fig:merged-reuse-count}
% \end{figure}




\mypar{(3)~Skewed expert reuses can enhance caching}
In autoregressive LLM tasks, MoE models exhibit skewed expert reuse across iterations, as our analysis of real-world data in Figure~\ref{fig:expert-reused} shows. Sampling two LLM requests, we observed distinct reuse patterns; for instance in sequence 1, in Mixtral's last layer, Expert 2 was reused over 15 times, and 7 times far more than others. 
In Sequence 2, Expert 0 had the highest reuse count, followed by Expert 5, both considerably exceeding others.
Similarly, in NLLB, fewer than 10\% of experts are activated, with a select few, like Expert 126, being heavily reused.

% \review{
% During decoding iteration, the expert activation pattern is low in correlation between each iteration, while exhibit skewed expert reuse on a few experts.
% As shown in Figure~\ref{x}, we sample over 1000 sequences for each dataset and model and compute the Pearson correlation within decoding phase for each input sequence. 
% We observe that the patterns are largely not repeating and similar across iteration, showing low correlation (X on average) across most samples.
% Further, we demonstrate the cumulative expert activation for all iterations for a given sequence in Figure~\ref{x} as heatmap.
% A clear stripe for each sequence shows the skewed reuse, with X-Y\% of the iteration is routed through the highlighted experts.
% }

The skewed reuse of experts becomes more uniform across multiple requests. After analyzing over 1000 sequences with Mixtral, expert reuse counts even out. NLLB shows a similar trend, albeit less pronounced than in single-request scenarios. This suggests the potential for improved cache performance by leveraging skewed reuse patterns in each sequence. By prioritizing heavily reused experts, we can optimize cache footprint and replacement strategies to enhance cache hit ratios, utilizing idle High Bandwidth Memory (HBM) on GPUs post-inference runtime initialization.



\begin{comment}
\subsection{Open Concerns}
\label{sec:open-concerns}

Based on the design intuitions above, we aim to enable expert activation awareness in MoE serving systems, focusing on tracing the expert's selective activation, group activation, and skewed reuse during inference. Leveraging this trace, this serving system can effectively prefetch and cache experts in GPUs, maximizing efficiency in supporting offloading.

To realize such a system design, two open concerns must be addressed:

\mypar{(1) New methods for tracing expert activation}
We need methods to trace the expert activation. These methods must trace various information, including those related to (i)~the selective activation of experts, (ii)~the group activation of experts on multiple layers, and (iii)~the skewed reuse of experts at the request level. 
Current tracing approaches, used in BrainStorm and DeepUM, cannot effectively provide the above information. They adopt a conceptually model-level expert tracing approach where the expert's usages are accumulated across all requests since serving the model. They thus suffer from the uniform distribution of expert activation emerging at the model level, thus falling short in effectively guiding prefetching and caching decisions based on their historical traces.
\review{
Tracing at finer granularity imposes additional requirement on the runtime efficiency and memory space complexity for scalability in large MoE models.
}




\mypar{(2) New methods for expert prefetching and caching}
New methods for prefetching and caching experts are needed. When operating an MoE model, the activation information, including expert selection, group activation, and reuse, is continuously updated. This necessitates the inference runtime to dynamically adjust its prefetching and caching priorities. For instance, an expert initially predicted for activation and thus prefetched might later be deprioritized based on new activation data. Additionally, the runtime should consider the MoE model's architectural characteristics. For example, activation predictions may vary in accuracy; layers closer to the active layer typically offer more precise predictions than those farther away. This factor should be considered when setting prefetching priorities. Prefetching and caching are interdependent; prefetching may not benefit the initial layers as much, so caching should prioritize likely activated experts in these layers. These considerations are also crucial in the cache replacement strategy.
\end{comment}



==> sections/prefetch-cache.tex <==
\section{Prediction-Guided Prefetching \& Caching}
\label{sec:eap-inference-runtime}

% In this section, we describe how \sys leverages the expert activation trace (stored in EAMC) to achieve effective prefetching and caching in a multi-GPU server. 

\subsection{Expert Prefetching Strategy}
\label{sec:expert-prefetching-strategy}
% \todo{prefetching implementation - coordinator + per-link worker and queues, prefteching priority}
 
We aim to design an expert prefetching strategy that meets two key objectives: (i) The prefetching operation for an expert should commence timely so that by the time the GPU requires this expert, it is already fully available in the GPU prefetching buffer, thereby minimizing the duration the GPU is blocked. (ii) The prefetching operations must also minimize the consumption of valuable PCIe bandwidth. This means that prefetching should be limited to experts that will actually be used, avoiding unnecessary prefetching of unused experts as much as possible. 
% \yao{I thought section 4's contribution decides the prefetching targets. No?}

\mypar{Intuitions for enhancing prefetching} To optimize prefetching bandwidth, our intuition is to use the iEAM. By matching the iEAM with historical ones in the EAMC, we identify similar past EAMs that help predict which experts might activate in subsequent layers. This allows us to prefetch only those experts, thereby saving bandwidth.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/illustration/prefetch_baselines.pdf}
    \caption{Prefetching examples.}
    \label{fig:prefetch-baselines}
\end{figure}

Further, to enhance the timeliness of prefetching, our intuitions include: (i)~We extend prefetching to multiple layers, termed multi-layer prefetching, enabling timely readiness of experts that are likely to activate even several layers ahead. This approach is particularly beneficial for emerging MoE models with different TopK activation.
% , such as QWen-60x1B, which feature a permanently active expert per layer. \yao{In this case, why not treat these experts just as dense modules?} 
(ii)~We prioritize experts based on their proximity to the current layer, giving higher prefetching priority to nearer experts due to their sooner usage and the greater impact of their absence on GPU utilization. 
(iii)~Experts that fail to be prefetched are assigned the highest prefetching priority to jump over prefetched experts in the PCIe queue, further minimizing GPU blocking time.

\mypar{Prefetching examples} We demonstrate how integrating our insights can enhance prefetching effectiveness over existing strategies, as depicted in Figure~\ref{fig:prefetch-baselines}. Consider a scenario where an MoE model completes the first layer and proceeds to the second. Once a token is dispatched to E[2,1], the dependency-based strategy (implemented in DeepSpeed-Inference) begins prefetching E[3,1] and E[3,2] in the immediate next layer (shown in (a)). However, when the output of E[2,1] is later routed to E[3,2], the parameters for E[3,2] are not ready in the GPU's buffer, causing the GPU to be blocked. 
% \yao{You might want to introduce fig 7 (a) as well. Similarly for following text, mention fig 7 (b,c) at the right place.} 
This blocking issue can be seen for E[4,2] again.

% The correlation-based strategy (shown in (b)), used in BrainStorm and DeepUM, could leverage correlation counts to tell E[3,2] is used more frequently than E[3,1], and it thus prioritizes E[3,2] and let it be ready sooner. Once it knows only E[3,2] is needed, the prefetching of the unused E[3,1] can be canceled to save bandwidth. Despite this improvement, the correlation counts often yield a uniform distribution across experts, failing to provide a clear differentiation. 
The model-level tracing strategy (shown in (b)), used in BrainStorm and DeepUM, could leverage model-level counts to tell E[3,2] is used more frequently than E[3,1], and it thus prioritizes E[3,2] and let it be ready sooner. Once it knows only E[3,2] is needed, the prefetching of the unused E[3,1] can be canceled to save bandwidth. Despite this improvement, the model-level counts often yield a uniform distribution across experts, failing to provide a clear differentiation. 
This leads to situations where both E[4,1] and E[4,2] are prefetched without appropriate prioritization, still causing GPU blockage for E[4,2]. Note that the issue of the uniform counts is rising with the number of experts per layer, ultimately resulting in poor prefetching effectiveness, detailed in Section~\ref{sec:eval-expert-prefetching}.

The strategy (shown in (c)) that combines all our above design intuitions can correctly predict E[3,2] and E[4,2] are more likely to be activated than E[3,1] and E[4,1] through EAM-based activation prediction and multi-layer prefetching. It further knows that E[3,2] is sooner to be used than E[4,2] (through prioritizing layers based on proximity). Hence, this strategy achieves the best prefetching performance in this example.

\mypar{Prefetching process} We describe the process that implements our prefetching strategy. The prefetching process initializes the GPU with a fixed-size buffer where each slot corresponds to an expert. After knowing the routing decisions in each MoE layer, there is an I/O thread computes the latest prefetching priorities for all experts in the subsequent layers. Based on the new priorities, it adjust its current prefetching operations. Additionally, the I/O thread avoids contention on PCIe bandwidth. When multiple experts are needed for prefetching, they flow through the PCIe connection sequentially.
The priority of prefetching is based on the predicted activation likelihood.

% We define the prefetching priority computation and illustrate its computation process in.
% Figure~\ref{fig:probability-compute} revisits the MoE model from Figure~\ref{fig:prefetch-baselines}. After R2 finishes dispatching the token to E[2,1], we need to adjust the order of prefetching.
% For this, \sys utlizes iEAM that traces the numbers of tokens passing through different experts in the current iteration.
% This iEAM is matched with prior EAMs in the EAMC (shown in \myc{1}). Several matched EAMs might be returned. In such a case, we aggregate them and compute activation probability for each expert possiblly to activate (shown in \myc{2}).
% In this aggregation step, formally, the cell of each matched EAM is summed up and normalized on each row. To ensure future experts in proximity to the current layers can be prioritized, the layer proximity step (shown in \myc{3}) adjusts the value in each cell through the formula $(1-(i-l)/L)$, where $l$ is the current layer ID and $i$ is the future layer ID. This design fixed the issue in Figure~\ref{fig:prefetch-baselines} where $\E32$ needs to be prefetched first than $\E42$ even though it shows a lower activation probability purely based on EAM analysis. 

The I/O thread can also handle the contention for the slots in the GPU buffer. When the buffer is full, it will compare the current top-K most important experts to prefetch (where K is the total number of slots in the buffer). For those already in the buffer, we skip their prefetching. For those not in the buffer, we start their prefetching into the slots that exhibit lower priorities.


\subsection{Enhancing Expert Prefetching with Caching}

We aim to enable effective caching for the experts that have been loaded into the GPUs. Thus, if they are reused in the next iteration, they can be immediately accessed within the GPUs, reducing the need for repetitive fetching. To facilitate this, we have enhanced the GPU buffer with extra caching capabilities. 

For consolidating caching and prefetching operations, the buffer now implements the following mechanisms:
(i) It provides slots to hold the experts being prefetched (or fetched on-demand) into the GPU,
(ii) It assigns idle slots (those not currently used for fetching) to cache previously used experts,
(iii) When the cache is full and an additional slot is needed for prefetching, we examine all being cached experts and replace the one that shows the lowest cache priority (\ie given by the rEAM).
% \yao{Same thing as the last paragraph of 5.1?} 
In this cache replacement process, we need to protect being prefetched experts from eviction.
% \yao{Is this the priority over PCIe link? If an expert is already cached, why would it be transferred again?} 
The primary reason is prefetched experts need to be used sooner by the GPU. They are more likely to be used compared to the cached ones which have been used in this iteration and are cached to benefit future reuses. For this, being prefetched experts are given maximal cache priorities until they are used or their corresponding layers have passed in the current iteration.

\mypar{Intuitions for combing caching with prefetching} 
% \yao{What is a rEAM?}
When integrating caching with prefetching, we want to maximize the buffer hit ratio (\ie buffer is regarded as a hit if the expert is cached locally or has been prefetched fully when activated). For this, we have two novel intuitions. First, we use the count of rEAM to reset an expert's priority in the buffer after it has been used by the GPU or determined not to be called in this iteration (i.e., a mis-prefetching case). 
% \yao{The entire paragraph is not very clear to me.}

Our second intuition addresses the initial layers of MoE models, which typically benefit less from prefetching due to less confident prediction of the group activation pattern at the start. By assigning higher caching priorities to experts in these initial layers, we not only counteract potential prefetching failures but also exploit the layer-by-layer execution property of MoE models: the subsequent layers are executed later and they are more likely to benefit from prefetching and thus less need caching.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/illustration/cache_example.pdf}
    \caption{Example of integrating caching with prefetching.}
    \label{fig:cache-example}
\end{figure}

\mypar{Examples of integrating caching with prefetching} 
Figure~\ref{fig:cache-example} shows how to intergrate caching with prefetching enhances caching effectiveness. In the second iteration, the cache strategy influences the initial layers. Augmenting dependency-based prefetching with an LRU cache, as in DeepSpeed-Inference, prefetching $\E21$ evicts $\E31$, leading to a buffer miss when tokens route to $\E22$ (see (a) left). For model-level tracing with LRU, as in DeepUM and BrainStorm, uniform activation means $\E11$ could route to $\E21$ or $\E22$, resulting in a buffer miss (see (b) left). Our method, using a rEAM $[[1,2], [0,3], [0,3]]$, keeps $\E22$ from eviction, ensuring a buffer hit and better latency (see (c) left).

At layer 3, prefetching's role intensifies. Dependency-based prefetching misses $\E32$, causing a buffer miss (see (a) right). Model-level tracing identifies the layer 3 expert but risks future misses by evicting $\E22$ (see (b) right). Our strategy accurately prefetches and retains $\E22$, preventing its eviction and optimizing cache prioritization (see (c) right).


\mypar{Priority update mechanism} We introduce a dynamic priority update mechanism for experts in the buffer, enhancing our caching and prefetching strategy. Upon prefetching, an expert's priority is initially set to maximum. The expert priority will be reset to rEAM based on three scenarios: (i) when expert finishes its inference. (ii) unused experts already prefetched after token dispatching. (iii) Prefetched experts not among the top-K per GPU.



